INFER: INtermediate representations for FuturE pRediction

In urban driving scenarios, forecasting future trajectories of surrounding vehicles is of paramount importance. While several approaches for the problem have been proposed, the best-performing ones tend to require extremely detailed input representations (eg. image sequences). But, such methods do not generalize to datasets they have not been trained on. We propose intermediate representations that are particularly well-suited for future prediction. As opposed to using texture (color) information, we rely on semantics and train an autoregressive model to accurately predict future trajectories of traffic participants (vehicles) (see fig. above). We demonstrate that using semantics provides a significant boost over techniques that operate over raw pixel intensities/disparities. Uncharacteristic of state-of-the-art approaches, our representations and models generalize to completely different datasets, collected across several cities, and also across countries where people drive on opposite sides of the road (left-handed vs right-handed driving). Additionally, we demonstrate an application of our approach in multi-object tracking (data association). To foster further research in transferrable representations and ensure reproducibility, we release all our code and data.

==> 07acknowledgements.tex <==
\section*{Acknowledgements}

We thank Ondrej Miksik (Oxford University) and Vibhav Vineet (Microsoft Research, Redmond) for helpful discussions during the course of this project. We also thank Prakyath, Sidhant, Viswa and Shubham for manually annotating several sequences from the Cityscapes dataset.


==> 08DiscussionandFuture.tex <==
\section*{Discussion}

Learning a suitable representation from the dataset makes the whole point of transferablity moot as the learned representation would again be dependent on the dataset it was learned from, hence defying the whole idea of transferablity. These learned representations would prove out to be insignificant when faced with a new dataset. On the other hand, the proposed representation is agnostic to the dataset and can be incorporated in any future trajectory prediction problem. It is simple and easy to compute rather than relying on complex handcrafted features. 
Future work can look at trying to learn representations that are data agnostic. Predicting future semantics to aid the prediction of future locations can also be looked at.

